Achieving Linear Speedup in Non-IID Federated Bilevel Learning

Federated bilevel optimization has received increasing attention in various emerging machine learning and communication applications. Recently, several Hessian-vector-based algorithms have been proposed to solve the federated bilevel optimization problem. However, several important properties in federated learning such as the partial client participation and the linear speedup for convergence (i.e., the convergence rate and complexity are improved linearly with respect to the number of sampled clients) in the presence of non-i.i.d.~datasets, still remain open. In this paper, we fill these gaps by proposing a new federated bilevel algorithm named FedMBO with a novel client sampling scheme in the federated hypergradient estimation. We show that FedMBO achieves a convergence rate of $\mathcal{O}\big(\frac{1}{\sqrt{nK}}+\frac{1}{K}+\frac{\sqrt{n}}{K^{3/2}}\big)$ on non-i.i.d.~datasets, where $n$ is the number of participating clients in each round, and $K$ is the total number of iteration. This is the first theoretical linear speedup result for non-i.i.d.~federated bilevel optimization. Extensive experiments validate our theoretical results and demonstrate the effectiveness of our proposed method.

==> minhui_draft/FedetatedBilevelLinearSpeedup-4/.git/objects/52/b27516942e1d2b7a5d40175b1f71ee2a324dbf <==
x]'Ñnà E÷ÌW\©¯mH3U}އÔIèŠF Úi?;¡U7?0ßcgðq@ߛ·ÍT(ۂ\Òm,·d•ÚpÚ¹I©Ü<§0Ú	‰Š‹h›Vã½m[Ü3Y¢y?zgCÉ[X/õ"eèý™æ«·|©õ%'[tüž<¿N¦8ûŸªúSàœâüJ0­¨+`ˆaW!ÙÀ"Þm"ïQE`s¹þÇwv)s¯1ˆ¸¢áەÊźOƒõ˧€|õ®ÈvF‰0Üéàãø•e›ÏFN'¥ŸaÑIì%ú¾_ּܺÉÒAT{™åì>LuzLVpã­ Ù«§ÑÎ<ûO¢õg@WW±Q5g$Çþ‹aÍuÇGHºý'3Kéò¥|

==> minhui_draft/FedetatedBilevelLinearSpeedup-4/.git/objects/54/c82dd8bc39eef41523ab3e2b2b076c85784c4f <==
x]RÝo›0ß³ÿŠSžZ	uí&uo˜ÆÁÈ8Íòȇ<a³¬ÿýÎ$iµIHÈç»ß×¹îm
O_Ÿ?­¹'Ì4zpšØžÞFsè<Ü5÷ðåñéÊ®²ŒðÝRèñhœÃ3uý‡±¼n#؏ZƒÝCÓUãAGà-TÃœôèpÀÖ¾2ƒA¤
$"Øé;"qvïÏÕ¨±¹…Ê9ۘ
ñ µÍtԃ¯|àۛ^;¸ó†EyXÜÏ$­®zbDÓp»'³ñ<ŒÚùÑ4#34ýÔ
·ëÞ͕!ŒÏîAå"CAgGۚ}øëÙÖiª{ãºZ ëÉc§Å9Æ(øølGpºï	"Ô={ýP7÷"|0ä¿FäBåÜÙã¿NŒ#ûiCÁŽÖbd3ã/ÝøP	Ê÷¶ïí9XkìКà×}#DáUUÛßzörYî`=Jãž0‹¸lõz庪ï¡Ö×ÀãÅÒ»t7ÕÎãâMÕÃɎ3ßÿ6Å ©ÚRɀ—PHñÊ–À'–x^D°åj%6
°CÒ\í@¤@óüàyûYHV– $áë"ãk<³MÂóXâ\.ðs|ǪÂ+g8—šÉx…ÈtÉ3®vI¹Êf*$P(¨T<ÞdTB±'…(Ò'›ó<•ÈÂÖ,WȊ5`¯x€rE³,PºAõ2èƒX;É_V
V"K—•ÑeÆ.Th*Î(_GÐ5}	ê$D'$´]ÔÁvÅB)ðQübÅElÄ"Wº"ê}tËK•¼¤R¬#âÄ	DGœËÙ%D=ô¾l	mÐôM$Œfˆ…ëÉg‹·æò"WVú

==> minhui_draft/FedetatedBilevelLinearSpeedup-4/.git/objects/d6/44681d86f46f04460643af813a2b412b87214b <==
x]TKo1?6YBZ^PT*Ä©'*‐Ï
$"ªJ­@Ñvm'
›dk;} Í	®üɑ?ÄÁWNüNÌxËCxå±=ö|ö|ói÷ŠÉÞµ[·n߅ÇKK-ÀÖkfßÀwZün'±Û-4
+ ¡'lÄÎjŸHúD!F2'è"*úI¤ª‰cCÅêŽMÅ^B§õ'`»Ã|¤Üq©qÂÇ㌑›ÄÞÄþ»-Ð8˜³
/^…›±£×›ólÁÛ3~tÃ	ŝ¬à#ûÈÑ·6«x«PA%ÐòU¸îÁþæ.¸hÞ ýU¨cœV¸wy*zœØ6ôd:M/³Iyìc¥ufò½>¶>2鸯½(ôØGnb²*?èHÏ}tØKúž½÷,ÿ
æ,ý|Ð}eµ±ÝÁGùx0Í»["l:Òcg»F["H¯4"a÷©VÛÚºîÔ入Õ
|AÇGýÓfÛh€-ã·ÂÖð3çqQ¨}ö@ßNOèr"±¦rˆ4
¥âŸ'¸Rm¤ŽWâÌøþRó¨â®AÔ.ø¼¹@ÅÿRÔá†îô
¥òLwbC"òÑm&H'¤¥'Ìôzº9uàÒlБ†2ñ25}k–h{™V›s´Ý¬3ß!dÊ®³kcòæ2úþ膒þ£›/¸pà0qÔ©f£N›PX}LweÆŸcÊCYa'ïÉýõ]8zã"%N"IQÏgâh‹h±'ñµ¶~£å­¿á3>""pe{	ˆÈã]ØŠ(H¢¬uæejґ5T6Ô[ô®˜¤.ðè´yÙ7©21ñâC^v¢¤EÛ+rë'Öx:êeEŽZJxyӜÁs‰$Üÿ¹\®¹|†±tú
´Ä9°6¿ˆ"®°M¶.ÌUô`9‰P!xy\בØ7ø€ ¸À~8ûÏ5¡x¡nñ½ÑDM}Ÿ`'fc,vÇqósdòº

==> minhui_draft/FedetatedBilevelLinearSpeedup-4/.git/objects/fb/435d334762c87e9aa3ddfa0991bb6436060c2f <==
x+)JMU022d040031QHËL7Ô+ÈKg¸ÂväeíÃ{e¹6'V56ñXLž(œ€PcVkú!æõ·<)Õ¥+ö|>rþ©Ú|"c°šâíO¦=y*x®6ó«è3"ög=̑Ô@,3ºR½S2pÆŌ©Z‡¤ÞìpÚ!ò?¡ÈlÐ翲æwžeé'ž\PºiåÒx"X"šøĜô|°º)ùG6œV²nšþs½îŸ'»þ[˜•>]¥

==> minhui_draft/FedetatedBilevelLinearSpeedup-4/.git/objects/fc/f5ab7773013f6b89e3bdaae369340ed269d97c <==
x}RÛjÃ0Ýs¾BdŒ&4éÃ`¼/ûRŒ›8ÁàØ!vwaìßgٮӌQ?	IÇ:çH'©Oð¼{ºã¤g_l"YÖJf¼êaàsQî3p¯ã=P*"°"†Ë¾'^H®ØÈKx|7­xèÄnl¨/ur	üG©,õ`ÈwÞJÁ•5ùÇ
r;3¡¨Ô&fq¹åÆ^c'µí~•˜õYu¾ú"¾òìZW°|&M'ç
B
A] EE÷YûŽâä!Ã
b̆0¤ý¼èÙJê!)=Ölš¸êŠeFmµÆe™­Y¢I‡—íXlôB©–ÃYø¼6ŠV¢k½‰K&'\{cßÙŽú֒ºƒkkqA[²K2ìûõ\|/ú :ö?욆f¹Åhç·¦£¬`Ô'ùÇ6_âù×ÝyœB/ÚèÎ|©÷uëTò¢ü¸þ
